PAVEL: Decorative Patterns with Packed Volumetric Elements

Many real-world hand-crafted objects are decorated with elements that are packed onto the object's surface and deformed to cover it as much as possible. Examples are artisanal ceramics and metal jewelry. Inspired by these objects, we present a method to enrich surfaces with packed volumetric decorations. Our algorithm works by first determining the locations in which to add the decorative elements and then removing the non-physical overlap between them while preserving the decoration volume. For the placement, we support several strategies depending on the desired overall motif. To remove the overlap, we use an approach based on implicit deformable models creating the qualitative effect of plastic warping while avoiding expensive and hard-to-control physical simulations. Our decorative elements can be used to enhance virtual surfaces, as well as 3D-printed pieces, by assembling the decorations onto real-surfaces to obtain tangible reproductions.

==> Pipeline.tex <==
\section{PAVEL pipeline}
\label{sec:pipe}
%\textcolor{red}{Explain again what we want to do, placing the objs, having some intersections, deform them preserve the volume, revert to smooth mesh again.}

Figure \ref{fig:decopipeline} shows the proposed design pipeline provided by our system. The aim is to allow users to easily create a variety of our element-based artistic relief patterns over arbitrary base surfaces by controlling a few parameters in a simple way. The method should work with sufficiently complex background surfaces and non trivial decorative elements, providing a reasonably good simulation of a real deformable packing of clay-like material.
The main ingredients of the pipeline are:

\begin{itemize}
\item a method able to take an initial configuration of partially overlapping volume elements and transforming it in a set of non-overlapping, plastically deformed elements attached to the base and preserving the original volumes
\item a set intuitive parametric functions able to create initial configuration of elements with the right amount of overlap to create different type of patterns with simple and easily learned choices.
\end{itemize}

In the following subsection we describe the methods and options implemented in PAVEL for the two main tasks, then we will discuss \filippo{what?}

%The quick creation of a decoration made of deformed volumetric elements over a base surface requires two main ingredients: a method to sample initial positions for the elements in a controlled way at approximately fixed distances creating small intersections between them and possibly designing meaningful patterns, and a method to create the simulated crushing of the elements with each other.
%The proposed decoration pipeline is shown in Figure \ref{fig:decopipeline}.
%In the following subsection we describe the methods and options implemented in PAVEL for the two main tasks, starting from the packing solution simulating the





